Open-Vocabulary Temporal Action Localization using Multimodal Guidance

Open-Vocabulary Temporal Action Localization (OVTAL) enables a model to recognize any desired action category in videos without the need to explicitly curate training data for all categories. However, this flexibility poses significant challenges, as the model must recognize not only the action categories seen during training but also novel categories specified at inference. Unlike standard temporal action localization, where training and test categories are predetermined, OVTAL requires understanding contextual cues that reveal the semantics of novel categories. To address these challenges, we introduce OVFormer, a novel open-vocabulary framework extending ActionFormer with three key contributions. First, we employ task-specific prompts as input to a large language model to obtain rich class-specific descriptions for action categories. Second, we introduce a cross-attention mechanism to learn the alignment between class representations and frame-level video features, facilitating the multimodal guided features. Third, we propose a two-stage training strategy which includes training with a larger vocabulary dataset and finetuning to downstream data to generalize to novel categories. OVFormer extends existing TAL methods to open-vocabulary settings. Comprehensive evaluations on the THUMOS14 and ActivityNet-1.3 benchmarks demonstrate the effectiveness of our method. Code and pretrained models will be publicly released.

==> sec/02_relatedwork_style1.tex <==
\section{Related Work}
\label{sec:related_work} 
% need to reduce to 1 page
\vspace{-0.2cm}
% Do not start a section immediately with a subsection. Either write a brief introduction to that section, or reorganize your document. 
\noindent \textbf{Temporal Action Localization:}~TAL aims to localize and recognize action categories in long untrimmed videos. Existing TAL methods fall into two categories: two-stage approaches, which involve proposal generation followed by classification (based on anchor windows \cite{buch2017sst,heilbron2016fast,escorcia2016daps}, action boundaries \cite{gong2020scale,lin2019bmn,lin2018bsn,liu2019multi,zhao2020bottom}, graphs \cite{bai2020boundary,xu2020g}, or transformers \cite{chang2022augmented,tan2021relaxed,awais2023foundational}), and single-stage approaches \cite{lin2021learning,zhang2022actionformer}, which are 
anchor-free are trained end-to-end. However, a key limitation of all current TAL methods is their closed-world assumption --- they require the same 
action categories, ranging from around 20 to 200, to be present in both training and inference, preventing generalization to novel action categories unseen during training. In contrast, our proposed method overcomes this limitation by enabling the localization and recognition of both base categories and novel action categories.

\noindent \textbf{Zero-Shot Temporal Action Localization:}~ZSTAL aims to localize and recognize novel action categories in untrimmed videos unseen during training. Traditional zero-shot learning approaches transfer knowledge from seen to unseen classes through shared semantic embeddings or vision-language alignments. Prior works can be classified into semantic embedding-based approaches such as ZSTAD \cite{zhang2020zstad}, TranZAD \cite{nag2023semantics} and vision-language model-based approaches such as  Efficient-Prompt \cite{ju2022prompting}, STALE \cite{nag2022zero}, and ZEETAD \cite{phan2024zeetad}. However, zero-shot methods still fall short of real-world applications, specifically because of the constraint of identifying unseen categories without prior knowledge and relying solely on the base categories. Our work introduces Open-vocabulary Temporal Action Localization, which focuses on learning from a larger available vocabulary dataset, allowing us to achieve 25\% mAP on novel action categories, compared to 10\% without any additional annotation.

\noindent \textbf{Prompt-based learning in computer vision:}~Prompt-based techniques have been widely used in the NLP domain \cite{jiang2020can,liu2023pre}. Prompting refers to designing an instruction which, when passed through the pretrained language model, can guide the downstream task. CLIP introduces prompt-based learning in image recognition tasks, where it shows learning relationships between vision-language models using large-scale image-text pairs. Several studies have extended CLIP to video understanding tasks such as pre-training[], video-text retrieval[], video recognition[], video captioning[], video grounding[], video question-answering[], they are limited to a fixed representation based on available classes during training. Furthermore, we make the first attempt to explore the emphasis of prompt template for extracting rich language descriptions and embeddings from the CLIP text encoder can benefit challenging downstream tasks such as localization.

In summary, while previous works like Efficient-Prompt, STALE and ZEE-TAD explore low-shot temporal action localization, we are the first to investigate the open-vocabulary setting. Our proposed approach leverages pretraining on a larger localization vocabulary dataset, fusing visual features with text descriptions from a language model to obtain rich multimodal representations. This allows the model to focus on visual cues and semantic context related to the actions, leading to improved performance on both base and novel action categories.

% Semantic embedding-based approaches, such as ZSTAD[], integrate the R-C3D framework to optimize activity label mapping through shared semantics between seen and unseen activities but depend on training with unseen semantic embeddings, which is impractical for real-world use. TranZAD [] uses semantic data from seen classes for training and introduces a network that links action visuals to specific semantic embeddings. 
% These studies rely on semantic embeddings such as Word2vec [] or Glove []. Vision-language model-based approaches, including Efficient-Prompt[], STALE [], and ZEE-TAD [], mark a transition to using large-scale pretrained ViL models, whose visual-textual alignment significantly surpasses previous ZSTAD methods, demonstrating ViL models' efficacy in agnostic action scenarios.
% \subsection{Zero-Shot Temporal Action Localization}
% Zero-shot Temporal Action Localization is designed to locate the moment when an unseen action occurs in untrimmed video. Traditional zero-shot learning approaches transfer knowledge from seen to unseen classes through shared semantic embeddings or vision-language alignments. Prior works can be classified into two categories: semantic embedding-based approaches such as  ZSTAD[] integrated the R-C3D framework to optimize activity label mapping through shared semantics between seen and unseen activities but depended on training with unseen semantic embeddings, impractical for real-world use. TranZAD [] used semantic data from seen classes for training and introduced a network linking action visuals to specific semantic embeddings. The above mentioned works relied on semantic embedding such as Word2vec [] or Glove []. Vision-Language model-based approaches such as, Efficient-Prompt[], STALE [], and ZEE-TAD []. These approaches mark a transition to using large-scale pretrained ViL models, whose visual-textual alignment significantly surpasses previous ZSTAD methods, demonstrating ViL models' efficacy in agnostic action scenarios. Zero-shot methods, however, are still not close to real-world application, specifically because of the constraint of identifying unseen categories without any prior knowledge and just relying on the base categories. This limitation has led to oversimplified approaches in some studies, where impractical conditions are assumed, like having access to test data during the training phase or annotations for unseen classes. Our work for the first time introduces Open-vocabulary Temporal action localization, which focuses on learning on larger available vocabulary data, allowing us to achieve 25\% mAP on novel action categories, compared to 10\%, without any extra annotation. 
% \subsection{Prompt-based learning in computer vision}
% Prompt-based techniques have been widely used in the NLP domain[]. Prompting refers to designing an instruction which, when passed through the pretrained language model, can guide the downstream task. For example, when a carefully curated prompt template is passed through GPT\-3.5[], it has shown great few-shot and zero\-shot generalization capabilities across various tasks. CLIP[] introduced prompt-based learning in image recognition tasks, where it showed learning relationship between vision-language models using large-scale image-text pairs. Some works have extended CLIP[] to video understanding tasks such as pre-training[], video-text retrieval[], video recognition[], video captioning[], video grounding[], video question-answering[] and so on. Although, all the above-mentioned approaches are progressing on learning the relationship between video-text representation. Yet, they are still prone to a fixed representation at training time based on the fixed classes available at that time, but focus on extending the learned multi-modality ( this word should also before) representation to open-world learning. Despite the progress in this area, there is no research in exploring the use of prompt-based learning for open-vocabulary temporal action localization tasks. Furthermore, we make the first attempt in addressing how putting emphasis on the prompt template and focusing on extracting richer descriptions from the CLIP text encoder helps with a challenging downstream task such as localization.

% In summary, while previous works like Efficient-Prompt [], STALE [], and ZEE-TAD [] explore zero-shot temporal action localization, they are still limited by the constraints of identifying unseen categories without prior knowledge and relying solely on base categories. Our work is the first to investigate the open-vocabulary setting for temporal action localization. Our proposed approach, OVFormer, leverages pretraining on a larger localization vocabulary dataset and introduces a Modality Mixer module that fuses visual features with rich text descriptions obtained from a language model. This allows the model to focus on background cues and objects causing the actions, leading to improved performance on both novel and base action categories. By learning from a larger available vocabulary and emphasizing the prompt template, OVFormer achieves significant gains in mAP on novel action categories compared to zero-shot methods, taking a step towards real-world applicability.

% To summarize, While the aformentioned works explore low-shot Temporal action Localization, to the best of our knowledge, we are the first to investigate Open-Vocabulary for Temporal Action localization. In this work, we propose a simple yet effective solution on how pre-training on a larger vocabulary localization dataset followed by enriching the text guidance by fusing in the visual features to get a rich description which when learned alonged with video features motivates the alogorithm to focus on objects that are causing the actions to occur. As a result, this results both quanititativly and qualitatively improve performance on novel and base+novel action categories. 
